Accelerating Aeroelastic UVLM Simulations by Inexact Newton Algorithms

We consider the aeroelastic simulation of flexible mechanical structures submerged in subsonic fluid flows at low Mach numbers. The nonlinear kinematics of flexible bodies are described in the total Lagrangian formulation and discretized by finite elements. The aerodynamic loads are computed using the unsteady vortex-lattice method wherein a free wake is tracked over time. Each implicit time step in the dynamic simulation then requires solving a nonlinear equation system in the structural variables with additional aerodynamic load terms. Our focus here is on the efficient numerical solution of this system by accelerating the Newton algorithm. The particular structure of the aeroelastic nonlinear system suggests the structural derivative as an approximation to the full derivative in the linear Newton system. We investigate and compare two promising algorithms based in this approximation, a quasi-Newton type algorithm and a novel inexact Newton algorithm. Numerical experiments are performed on a flexible plate and on a wind turbine. Our computational results show that the approximation can indeed accelerate the Newton algorithm substantially. Surprisingly, the theoretically preferable inexact Newton algorithm is much slower than the quasi-Newton algorithm, which motivates further research to speed up derivative evaluations.

==> abbr.tex <==
% Abbreviations -- requires package xspace

\newcommand\abbrfont{}

\newcommand\abbr[1][abbrev]{{\abbrfont{#1.}}\xspace}
\newcommand\abbrev{\abbr}
\providecommand\ca{\abbr[ca]}% Also in abk.tex.
\newcommand\cf{\abbr[cf]}
\newcommand\eg{\abbr[e.g]}
\providecommand\etal{\abbr[et~al]}% Also in abk.tex.
\providecommand\etc{\abbr[etc]}% Also in abk.tex.
\newcommand\ie{\abbr[i.e]}
\newcommand\resp{\abbr[resp]}
\providecommand\vs{\abbr[vs]}% Also in abk.tex.
\newcommand\Wlog{\abbr[w.l.o.g]}% \wlog is an internal logging command.
\newcommand\wrt{\abbr[w.r.t]}


==> abk.tex <==
% Abkürzungen -- benötigt package xspace

\newcommand\abkfont{}

\newcommand\Abk[1][Abk]{{\abkfont{#1.}}\xspace}
\newcommand\bzw{\Abk[bzw]}
\newcommand\bzgl{\Abk[bzgl]}
\providecommand\ca{\Abk[ca]}% Also in abbr.tex.
\let\TeXdh\dh
\renewcommand\dh{\Abk[d.\,h]}% Now \dh, not \ie: original \dh mostly unused.
\PackageInfo{abk}{Redefining \string\dh\space
 (use \string\TeXdh\space for TeX \string\dh)}
\providecommand\Dr{\Abk[Dr]}
\providecommand\DrIng{\Abk[Dr.-Ing]}
\newcommand\engl{\Abk[engl]}
\providecommand\etal{\Abk[et~al]}% Also in abbr.tex.
\providecommand\etc{\Abk[etc]}% Also in abbr.tex.
\newcommand\evtl{\Abk[evtl]}
\newcommand\ggf{\Abk[ggf]}
\newcommand\iA{\Abk[i.\,A]}
\newcommand\MEd{\Abk[M.\,Ed]}
\newcommand\MSc{\Abk[M.\,Sc]}
\newcommand\OBdA{\Abk[O.\,B.\,d.\,A]}
\newcommand\oBdA{\Abk[o.\,B.\,d.\,A]}
\newcommand\oE{\Abk[o.\,E]}
\newcommand\og{\Abk[o.\,g]}
\providecommand\Prof{\Abk[Prof]}
\newcommand\sog{\Abk[sog]}
\newcommand\ua{\Abk[u.\,a]}
\newcommand\usw{\Abk[usw]}
\newcommand\vgl{\Abk[vgl]}
\newcommand\wiss{\Abk[wiss]}
\providecommand\vs{\Abk[vs]}% Also in abbr.tex.
\newcommand\zB{\Abk[z.\,B]}
\newcommand\zT{\Abk[z.\,T]}


==> bridge.tex <==
This example is taken from \cite{?} where it was designed
to conduct a nonlinear aeroelastic analysis of a cantilever plate,
with a focus on flapwise and torsional motion
The structural parameters are derived from Fung's suspension bridge model
presented in \cite{fung1955}.
These parameters include a chord length of $c = \SI{60.0}{ft}$,
a squared gyration ratio of $r_\alpha^2 = 0.6222$,
mass density per unit length at $m = \SI{269.0}{slug/ft}$,
a natural bending frequency of $\omega_h = \SI{0.88}{rad/s}$,
and a natural torsion frequency of $\omega_\alpha = \SI{1.55}{rad/s}$.

In our aeroelastic model,
we employ the vortex lattice method for aerodynamics,
and the structure is represented as a collection
of geometrically exact beam elements.
To adapt Fung's one-dimensional model
to our three-dimensional geometrically exact model,
we determine the elastic properties needed to achieve identical
torsional and bending eigenfrequencies for the cantilever.
The structural configuration comprises a constant rectangular cross-section
with isotropic linear elastic material properties.
This includes a Young's modulus of $E = \SI{1.936e7}{lbf/ft^2}$,
a shear modulus of $G = \SI{7.840e4}{lbf/ft^2}$,
and a material density of $\rho = \SI{8.027e-2}{slug/ft^3}$.
Consequently, the cross-sectional dimensions
have a chord length of $c = \SI{60.0}{ft}$
and a thickness of $t = \SI{55.85}{ft}$.
It is important to note that the thickness $t$
does not correspond to that of a thin plate.
However, this choice was made to replicate the desired structural behavior,
primarily focusing on flapwise and torsional motions
while minimizing edge-wise motion.
Additionally, we mitigate the impact of shear deformations
by introducing sufficiently high shear stiffness
with $GA_1 = GA_2 = \SI{1.0e12}{lbf\,ft^2}$,
along with a cantilever length of $L = \SI{1000.0}{ft}$.
The air density is given as $\rho_F = \SI{2.378e-3}{slug/m^3}$.
A summary of the geometric and material input data
for both the structural and aerodynamic models
is given in \cref{tab:ex02_main_geometry}.
%
\begin{table}
  \centering
  \caption{Geometry and material parameters for beam model.}
  \label{tab:ex02_main_geometry}
  \begin{tabular}{lr}
    \toprule
    Parameter & Value \\
    \midrule
    Length $L$    & \SI{1000.0}{ft} \\
    Chord $c$     &   \SI{60.0}{ft} \\
    Thickness $t$ &  \SI{55.85}{ft} \\[\jot]
    Fluid density $\rho_F$  & \SI{2.378e-3}{slug/m^3} \\
    Young's modulus $E$     &  \SI{1.936e7}{lbf/ft^2} \\
    Shear modulus $G$	    &  \SI{7.840e4}{lbf/ft^2} \\
    Material density $\rho$ & \SI{8.027e-2}{slug/ft^3} \\
    \bottomrule
  \end{tabular}
\end{table}

The air inflow on the bridge deck is characterized by a free-stream velocity,
denoted as $V_\infty = \SI{190}{ft/s}$,
and an angle of attack, represented as $\alpha = \SI{5}{\degree}$.
In order to enhance convergence behavior
during the initial phases of the nonlinear calculation,
we avoid an abrupt start of the inflow
by implementing a linear factorization
of the vector of generalized aerodynamic forces.
Specifically, we incrementally increase the magnitude
of the aerodynamic forces until reaching the load step $T_d = 100$.
From that point onward, these forces are consistently applied
without alteration throughout the remainder of the simulation.
The simulation continues for a total of $T_n = 200$ steps
\emred{to ensure a steady-state solution}.
For the \emred{static} calculation, the influence of the wake
is considered within its \emred{steady-state} configuration.
To accurately capture the \emred{final} wake geometry,
the wake is convected within each simulation step
\emred{until a steady state is obtained}.
\emred{%
It is important to note that the path leading to the static solution
is solely of a numerical nature and does not represent a physical process.
}%
To mitigate the effects of singularities
resulting from vortex-induced velocities,
we introduce a cut-off value, denoted as $\delta = 0.01$.
The main simulation parameters are summarized in
\cref{tab:ex02_static_deformation_analysis_model_parameter}.
%
\begin{table}
  \centering
  \caption{Simulation parameters for
    nonlinear \emred{static} aeroelastic deformation analysis.}
  \label{tab:ex02_static_deformation_analysis_model_parameter}
  \begin{tabular}{lr}
    \toprule
    Parameter & Value \\
    \midrule
    Total number of load steps $T_n$ & \num{200} \\
    Cut-off radius $\delta$ & \num{0.01} \\
    FSI-influence radius $r_L$ & \SI{30.1}{ft} \\
    Angle of attack $\alpha$ & \SI{5.0}{\degree} \\
    Intensity of free-field velocity $V_\infty$ & \SI{190}{ft/s} \\
    Newton convergence tolerance tol$_N$ & \num{1e-6} \\
    \bottomrule
  \end{tabular}
\end{table}

The absolute tolerance for all three Newton algorithms is $10^{-6}$,
\ie, each iteration terminates when $\norm{F(y_k)} \le 10^{-6}$.
For the inexact Newton algorithm we consider three different forcing sequences,
\begin{align*}
  \eta_k^1 &= \min\Bigl(\frac12, \norm{F(y_k}\Bigr),
  &\eta_k^2 &= 10^{-6} \eta_k^1,
  &\eta_k^3 &= 10^{-8} \eta_k^1.
\end{align*}
All three choices guarantee quadratic convergence.
The computational results are presented in \cref{tab:bridge:solvers},
where ``Inexact Newton $j$'' refers to forcing sequence $(\eta_k^j)$.
\begin{table}
  \let\mc\multicolumn
  \centering
  \caption{Solver statistics for aero-elastic simulation of bridge.}
  \label{tab:bridge:solvers}
  \ifcase0
  \begin{tabular}{l*5r}
    \toprule
    & Exact  & Quasi- & Inexact  & Inexact  & Inexact \\
    & Newton & Newton & Newton 1 & Newton 2 & Newton 3 \\
    \midrule
    \mc6c{\it Total} \\[1pt]
    Wall time & 2077.61 & 322.00 & 2176.70 & 1951.67 & 1835.62 \\
    Eval UVLM & 1797.66 &  77.23 & 1924.28 & 1700.32 & 1583.91 \\
    Eval structure & 0.643 & 0.664 & 0.698 &   0.613 &   0.573 \\
    Linear solver  & 33.92 & 2.782 & 2.999 &   3.221 &   3.276 \\[2pt]
    Newton steps   &   728 &   799 &   799 &     697 &     655 \\
    Refine steps   &   --- &   --- &   799 &    1945 &    2395 \\
    \midrule
    \mc6c{\it Average per time step} \\[2pt]
    Wall time      & 10.388 &  1.610 & 10.884 &  9.758 &  9.178 \\
    Eval UVLM      &  8.988 &  0.386 &  9.621 &  8.502 &  7.920 \\
    Eval structure & .00322 & .00332 & .00349 & .00307 & .00287 \\
    Linear solver  & .16962 & .01391 & .01500 & .01611 & .01638 \\[2pt]
    Newton steps   &  3.622 &  3.975 &  3.975 &  3.468 &  3.259 \\
    \bottomrule
  \end{tabular}
  \or
  \begin{tabular}{l*6r}
    \toprule
    & Exact  & Quasi- & Inexact  & Inexact  & Inexact & Inexact \\
    & Newton & Newton & Newton 1 & Newton 2 & Newton 3 & QN \\
    \midrule
    \mc7c{\it Total} \\[1pt]
    Wall time & 2077.61 & 322.00 & 2176.70 & 1951.67 & 1835.62 & 325.27 \\
    Eval UVLM & 1797.66 &  77.23 & 1924.28 & 1700.32 & 1583.91 &  77.73 \\
    Eval structure & 0.643 & 0.664 & 0.698 &   0.613 &   0.573 &  0.669 \\
    Linear solver  & 33.92 & 2.782 & 2.999 &   3.221 &   3.276 &  2.741 \\[2pt]
    Newton steps   &   728 &   799 &   799 &     697 &     655 &    799 \\
    Refine steps   &   --- &   --- &   799 &    1945 &    2395 &    799 \\
    \midrule
    \mc7c{\it Average per time step} \\[2pt]
    Wall time      & 10.388 &  1.610 & 10.884 &  9.758 &  9.178 &  1.626 \\
    Eval UVLM      &  8.988 &  0.386 &  9.621 &  8.502 &  7.920 &  0.387 \\
    Eval structure & .00322 & .00332 & .00349 & .00307 & .00287 & .00335 \\
    Linear solver  & .16962 & .01391 & .01500 & .01611 & .01638 & .01371 \\[2pt]
    Newton steps   &  3.622 &  3.975 &  3.975 &  3.468 &  3.259 &  3.975 \\
    \bottomrule
  \end{tabular}
  \emred{MCS: Inexact QN will possibly be removed!}
  \fi
\end{table}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> code-names.tex <==
% Code names -- requires packages xspace and relsize

\providecommand\sfnamesize{\relsize{0}}
\providecommand\sfname[1]{\textsf{\sfnamesize#1}\xspace}

\newcommand\plusplus{\raisebox{0.15ex}{++}}
\newcommand\ALADIN{\sfname{ALADIN}}
\newcommand\AMPL{\sfname{AMPL}}
\newcommand\BARON{\sfname{BARON}}
\newcommand\Bash{\sfname{Bash}}
\newcommand\BGL{\sfname{BGL}}
\newcommand\BLAS{\sfname{BLAS}}
\newcommand\Bonmin{\sfname{Bonmin}}
\newcommand\boost{\sfname{boost}}
\newcommand\Boost{\sfname{Boost}}
\newcommand\BoostMPI{\sfname{Boost.MPI}}
\newcommand\langC{\sfname{C}}
\newcommand\CC{\sfname{C\plusplus}}
\newcommand\Cpp{\CC}
\newcommand\CCEleven{\sfname{C\plusplus 11}}
\newcommand\CppEleven{\CCEleven}
\newcommand\CCFourteen{\sfname{C\plusplus 14}}
\newcommand\CppFourteen{\CCFourteen}
\newcommand\Clean{\sfname{Clean}}
\newcommand\clean{\sfname{clean}}
\newcommand\CleanIPM{\sfname{Clean::IPM}}
\newcommand\cleanIPM{\sfname{clean::ipm}}
\newcommand\CONOPT{\sfname{CONOPT}}
\newcommand\CONOPTfour{\sfname{CONOPT4}}
\newcommand\CPLEX{\sfname{CPLEX}}
\newcommand\CUTE{\sfname{CUTE}}
\newcommand\CUTEr{\sfname{CUTEr}}
\newcommand\CUTEst{\sfname{CUTEst}}
\newcommand\dealII{\sfname{deal.II}}
\newcommand\DeSiO{\sfname{DeSiO}}
\newcommand\DICOPT{\sfname{DICOPT}}
\newcommand\DOpElib{\sfname{DOpElib}}
\newcommand\DOM{\sfname{DOM}}
\newcommand\Doxygen{\sfname{Doxygen}}
\newcommand\EPANET{\sfname{EPANET}}
\newcommand\Excel{\sfname{Excel}}
\newcommand\FilterSQP{\sfname{FilterSQP}}
\newcommand\filtermpec{\sfname{filtermpec}}
\newcommand\GAMS{\sfname{GAMS}}
\newcommand\GasLib{\sfname{GasLib}}
\newcommand\GCC{\sfname{GCC}}
\newcommand\Gurobi{\sfname{Gurobi}}
\newcommand\Fortran{\sfname{Fortran}}
\newcommand\FortranSS{\sfname{Fortran 77}}
\newcommand\iGNO{\sfname{iGNO}}
\newcommand\Ipopt{\sfname{Ipopt}}
\newcommand\IPM{\sfname{IPM}}
\newcommand\Java{\sfname{Java}}
\newcommand\KNITRO{\sfname{KNITRO}}
\newcommand\KNITRODIRECT{\sfname{KNITRO/DIRECT}}
\newcommand\KNITROCG{\sfname{KNITRO/CG}}
\newcommand\LaGO{\sfname{LaGO}}
\newcommand\Lamatto{\sfname{LaMaTTO\plusplus}}
\newcommand\LAPACK{\sfname{LAPACK}}
\newcommand\Liwacom{\sfname{Liwacom}}
\newcommand\LOQO{\sfname{LOQO}}
\newcommand\MacMPEC{\sfname{MacMPEC}}
\newcommand\Matlab{\sfname{Matlab}}
\newcommand\MINLPLib{\sfname{MINLPLib}}
\newcommand\MINOS{\sfname{MINOS}}
\newcommand\MOSEK{\sfname{MOSEK}}
\newcommand\MPC{\sfname{MPC}}
\newcommand\MPI{\sfname{MPI}}
\newcommand\MSIPM{\sfname{MSIPM}}
\newcommand\MSKKT{\sfname{MSKKT}}
\newcommand\MSSQP{\sfname{MSSQP}}
\newcommand\MSTOP{\sfname{MSTOP}}
\newcommand\OOPS{\sfname{OOPS}}
\newcommand\openMPI{\sfname{Open MPI}}
\newcommand\Pardiso{\sfname{Pardiso}}
\newcommand\Python{\sfname{Python}}
\newcommand\SCIP{\sfname{SCIP}}
\newcommand\Simone{\sfname{SIMONE}}
\newcommand\SNOPT{\sfname{SNOPT}}
\newcommand\SQP{\sfname{SQP}}
\newcommand\TreeKKT{\sfname{TreeKKT}}
\newcommand\Xerces{\sfname{Xerces}}
\newcommand\XML{\sfname{XML}}
\newcommand\Zimpl{\sfname{Zimpl}}


==> math-fields.tex <==
% Math fields -- requires amsfonts

\newcommand{\field}{\mathbb}

% "natural" names
\newcommand{\complex}{\field{C}}
\newcommand{\quaternions}{\field{H}}
\newcommand{\naturals}{\field{N}}
\newcommand{\polynomials}{\field{P}}
\newcommand{\rationals}{\field{Q}}
\newcommand{\reals}{\field{R}}
\newcommand{\integers}{\field{Z}}

% alternative names
\newcommand{\numsetC}{\complex}
\newcommand{\numsetH}{\quaternions}
\newcommand{\numsetN}{\naturals}
\newcommand{\numsetQ}{\rationals}
\newcommand{\numsetR}{\reals}
\newcommand{\numsetZ}{\integers}

% short names
\makeatletter
\@ifundefined{C}{\newcommand{\C}{\complex}}
{\PackageInfo{math-fields}{Use \string\field{C} for complex numbers;
 \MessageBreak command \string\C\space already defined}{}}
\makeatother
\newcommand{\N}{\naturals}
\newcommand{\Q}{\rationals}
\newcommand{\R}{\reals}
\newcommand{\Z}{\integers}
\newcommand{\Poly}{\polynomials}% deprecated: NuMa scripts


==> math-std.tex <==
% Standard math definitions -- requires amsmath

\newcommand\const{\textup{const}}
\newcommand\qtext{\quad\text}
\newcommand\textq[1]{\text{#1}\quad}
\newcommand\qtextq{\quad\textq}
\newcommand\st{\textup{s.t.}}
\newcommand\stq{\st\quad}
\newcommand\qst{\quad\st}
\newcommand\qstq{\qst\quad}

\makeatletter
\newcommand\fcdot{\,\cdot\,}
\newcommand\ifgiven[3]{\def\fc@rg{#1}\ifx\fc@rg\empty#3\else#2\fi}
\newcommand\fcarg[1]{\ifgiven{#1}\fc@rg\fcdot}
\makeatother
\newcommand\abs[1]{\lvert\fcarg{#1}\rvert}
\newcommand\Abs[1]{\left\lvert#1\right\rvert}
\newcommand\tfracabs[2]{\abs{#1}/\abs{#2}}
\newcommand\fracabs[2]{\frac{\abs{#1}}{\abs{#2}}}
\newcommand\fracAbs[2]{\frac{\Abs{#1}}{\Abs{#2}}}
\newcommand\tabsfrac\tfracabs
\newcommand\absfrac\fracabs
\newcommand\Absfrac\fracAbs
\newcommand\card\abs
\newcommand\Card\Abs
\newcommand\ceil[1]{\lceil\fcarg{#1}\rceil}
\newcommand\Ceil[1]{\left\lceil#1\right\rceil}
\newcommand\pcolon{\mathpunct:}
\newcommand\defsep\pcolon% alternative: \mid
\newcommand\defset[3][\defsep]{\set{#2#1#3}}
\newcommand\Defset[3][\defsep]{\Set{#2#1#3}}
\newcommand\EEmult\cdot% alternative: \times
\newcommand\EE[1][\EEmult]{#1 10^}
\newcommand\floor[1]{\lfloor\fcarg{#1}\rfloor}
\newcommand\Floor[1]{\left\lfloor#1\right\rfloor}
\newcommand\Inv[1]{#1^{-1}}
\newcommand\HInv[1]{#1\ihr}% hermitian inverse
\newcommand\TInv[1]{#1\itp}% transpose inverse
\newcommand\norm[2][]{\lVert\fcarg{#2}\rVert\optsb{#1}}
\newcommand\Norm[2][]{\left\lVert#2\right\rVert\optsb{#1}}
\newcommand\tfracnorm[3][]{\norm[#1]{#2}/\norm[#1]{#3}}
\newcommand\fracnorm[3][]{\frac{\norm[#1]{#2}}{\norm[#1]{#3}}}
\newcommand\fracNorm[3][]{\frac{\Norm[#1]{#2}}{\Norm[#1]{#3}}}
\newcommand\tnormfrac\tfracnorm
\newcommand\normfrac\fracnorm
\newcommand\Normfrac\fracNorm
\newcommand\tfracnormpow[4][]{\norm[#1]{#2}^{#4}/\norm[#1]{#3}^{#4}}
\newcommand\fracnormpow[4][]{\frac{\norm[#1]{#2}^{#4}}{\norm[#1]{#3}^{#4}}}
\newcommand\fracNormpow[4][]{\frac{\Norm[#1]{#2}^{#4}}{\Norm[#1]{#3}^{#4}}}
\newcommand\pfrac[2]{\frac{\partial#1}{\partial#2}}
\newcommand\ppfrac[3]{\pfrac{^2#1}{#2\partial#3}}
\newcommand\set[1]{\{#1\}}
\newcommand\Set[1]{\left\{#1\right\}}
\newcommand\snorm[2][]{\lvert\!\lvert\!\lvert
  \fcarg{#2}\rvert\!\rvert\!\rvert\optsb{#1}}
\newcommand\Snorm[2][]{\left\lvert\!\left\lvert\!\left\lvert
  #2\right\rvert\!\right\rvert\!\right\rvert\optsb{#1}}
\newcommand\sprod[3][]{\langle\fcarg{#2},\fcarg{#3}\rangle\optsb{#1}}
\newcommand\Sprod[3][]{\left\langle#2,#3\right\rangle\optsb{#1}}

\newcommand\hrchar{H}
\newcommand\tpchar{T}
\newcommand\hr{^\hrchar}% hermitian transpose
\newcommand\tp{^\tpchar}
\newcommand\ihr{^{-\hrchar}}
\newcommand\itp{^{-\tpchar}}
\newcommand\tadj[1]{\mskip#1\thinmuskip}% adjust space
\newcommand\hra[1][0]{^{\tadj{#1}\hrchar}}
\providecommand\tpa[1][0]{^{\tadj{#1}\tpchar}}% Conflict with siamart190516.cls.
\newcommand\ihra[1][0]{^{\tadj{#1}{-}\hrchar}}
\newcommand\itpa[1][0]{^{\tadj{#1}{-}\tpchar}}
\newcommand\tpfrac[2]{\tfrac{\partial#1}{\partial#2}}
\newcommand\tppfrac[3]{\tpfrac{^2#1}{#2\partial#3}}
\newcommand\without{\setminus\set}
\newcommand\Without{\setminus\Set}

\newcommand\lbound{-}
\newcommand\ubound{+}
\newcommand\splb{^{\lbound}}
\newcommand\spub{^{\ubound}}
\newcommand\sblb{_{\lbound}}
\newcommand\sbub{_{\ubound}}
\newcommand\bounds[1]{\ensuremath{[#1\splb,#1\spub]}}
\newcommand\Bounds[1]{\ensuremath{\left[#1\splb,#1\spub\right]}}

\newcommand\Strut{\rule[2.5555ex]{0pt}{0pt}}% ~1.1em
\newcommand\Hline{\hline\Strut}

\newcommand\optsb[1]{\ifgiven{#1}{_{#1}}{}}
\newcommand\optsp[1]{\ifgiven{#1}{^{#1}}{}}
\newcommand\optindex[1]{\ifgiven{#1}{,#1}{}}
\newcommand\optmathsb\optsb
\newcommand\optmathsp\optsp
\newcommand\opttextsb[1]{\optsb{\textup{#1}}}
\newcommand\opttextsp[1]{\optsp{\textup{#1}}}
\newcommand\optmathindex\optindex
\newcommand\opttextindex[1]{\optindex{\textup{#1}}}

\newcommand\define{\mathrel{{\mathop:}{=}}}
\newcommand\enifed{\mathrel{{=}{\mathop:}}}


==> math-symbols.tex <==
% Math symbols -- requires amsmath

% Redefine some macros in math mode. Keep text mode definitions.
\let\TeXbar\_   % underscore -> \bar
\let\TeXhat\^   % undefined  -> \hat
\let\TeXtilde\~ % undefined  -> \tilde
\let\TeXcolon\: % \tmspace+\medmuskip{.2222em} -> \colon
\makeatletter
\newcommand\mcs@cc[3]{\leavevmode\ifmmode#1{#3}\else#2{#3}\fi}
\renewcommand\_{\mcs@cc\bar\TeXbar}
\renewcommand\^{\mcs@cc\hat\TeXhat}
\renewcommand\~{\mcs@cc\tilde\TeXtilde}
\renewcommand\:{\mcs@cc\colon\TeXcolon\relax}
\makeatother
\PackageInfo{math-symbols}{Redefining
 \string\_, \string\^, \string\~, \string\: in math mode.
 \MessageBreak Keeping text mode definitions.
 \MessageBreak Saving original commands as \string\TeXbar, \string\TeXhat,
 \MessageBreak \string\TeXtilde, \string\TeXcolon}

\newcommand\0\emptyset
\newcommand\bigM{M}
\newcommand\bigO{O}
\newcommand\smallo{o}
\newcommand\oo\infty
\newcommand\ox\otimes
\newcommand\x\times

\newcommand\itxt{\textup}% text in math indices
\newcommand\tsb[1]{_{\itxt{#1}}}% text subindex
\newcommand\tsp[1]{^{\itxt{#1}}}% text superindex

\newcommand\boundary\partial
\newcommand\cond\kappa
\newcommand\condabs{\cond\tsb{abs}}\newcommand\abscond\condabs
\newcommand\condrel{\cond\tsb{rel}}\newcommand\relcond\condrel
\newcommand\convrad\rho
\newcommand\eps\epsilon
\newcommand\veps\varepsilon
\newcommand\epsM{\veps\tsb{M}}
\let\epsmach\epsM
\newcommand\specrad\rho
\newcommand\spectrum\sigma
\newcommand\uvec{\mathbf1}

% Some arrows.
\newcommand\larrow\leftarrow
\newcommand\rarrow\to% \rightarrow
\newcommand\swap\leftrightarrow
\newcommand\lrarrow\swap
\newcommand\Larrow\longleftarrow
\newcommand\Rarrow\longrightarrow
\newcommand\LRarrow\longleftrightarrow
\newcommand\xlarrow\xleftarrow
\newcommand\xrarrow\xrightarrow
\newcommand\lArrow\Leftarrow
\newcommand\rArrow\Rightarrow

% Right-shifted relation symbols for alignment with :=
\newcommand\crel[1]{\mathrel{\hphantom:{#1}}}
\newcommand\isom{\crel\cong}
\newcommand\eqls{\crel=}


==> matrix.tex <==
% Matrices and column vectors -- requires amsmath

% Default space between array and delimiters.
\newcommand\matmargin{\,}
\newcommand\colmargin{\,}

% Separation lines.
\providecommand\vsl{|}
\providecommand\hsl{\hline}

% General delimited arrays: choose margin, format, delimiters.
% \Xmat{margin}{format}{ldelim}{rdelim}{entries}
\newcommand\Xmat[5][\matmargin]{%
  \left#3\begin{array}{@{#1}#2@{#1}}#5\end{array}\right#4}

% General matrices and vectors: choose margin, alignment, delimiters, ncol.
% ('<', '>' stand for ldelim, rdelim; last two args processed by \Xmat.)
% \xddmat[margin]{alignment}<nc1 nc2 nc3>{entries} (cols separated by |)
% \xdmat[margin]{alignment}<ncol1 ncol2>{entries} (cols separated by |)
% \xmat[margin]{alignment}<ncol>{entries}
% \xcol{margin}(alignment){entries}
\newcommand\xddmat[6][\matmargin]{
  \Xmat[#1]{*{#4}{#2}|*{#5}{#2}|*{#6}{#2}}{#3}}
% \Xmat[#1]{*{#4}{#2}\vsl*{#5}{#2}\vsl*{#6}{#2}}{#3}}
\newcommand\xdmat[5][\matmargin]{\Xmat[#1]{*{#4}{#2}|*{#5}{#2}}{#3}}
%\newcommand\xdmat[5][\matmargin]{\Xmat[#1]{*{#4}{#2}\vsl*{#5}{#2}}{#3}}
\newcommand\xmat[4][\matmargin]{\Xmat[#1]{*{#4}{#2}}{#3}}
\newcommand\xcol[3]{\Xmat[#1]{#3}{#2}}

% Standard matrices and vectors: choose alignment, delimiters, ncol.
\newcommand\lddmat{\xddmat[\matmargin]{l}}% \ldmat<nc1 nc2 nc3>{entries}
\newcommand\cddmat{\xddmat[\matmargin]{c}}% \cdmat<nc1 nc2 nc3>{entries}
\newcommand\rddmat{\xddmat[\matmargin]{r}}% \rdmat<nc1 nc2 nc3>{entries}
\newcommand\ddmat{\cddmat}
\newcommand\ldmat{\xdmat[\matmargin]{l}}% \ldmat<ncol1 ncol2>{entries}
\newcommand\cdmat{\xdmat[\matmargin]{c}}% \cdmat<ncol1 ncol2>{entries}
\newcommand\rdmat{\xdmat[\matmargin]{r}}% \rdmat<ncol1 ncol2>{entries}
\newcommand\dmat{\cdmat}
\newcommand\lmat{\xmat[\matmargin]{l}}% \lmat<ncol>{entries}
\newcommand\cmat{\xmat[\matmargin]{c}}% \cmat<ncol>{entries}
\newcommand\rmat{\xmat[\matmargin]{r}}% \rmat<ncol>{entries}
\newcommand\mat{\cmat}
\newcommand\col{\xcol{\colmargin}}% \col<alignment>{entries}


==> validation.tex <==
\one{Todo Z01: add established example for validation.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

